AV2Wav: Diffusion-Based Re-synthesis from Continuous Self-supervised Features for Audio-Visual Speech Enhancement

Speech enhancement systems are typically trained using pairs of clean and noisy speech. In audio-visual speech enhancement (AVSE), there is not as much ground-truth clean data available; most audio-visual datasets are collected in real-world environments with background noise and reverberation, hampering the development of AVSE. In this work, we introduce AV2Wav, a resynthesis-based audio-visual speech enhancement approach that can generate clean speech despite the challenges of real-world training data. We obtain a subset of nearly clean speech from an audio-visual corpus using a neural quality estimator, and then train a diffusion model on this subset to generate waveforms conditioned on continuous speech representations from AV-HuBERT with noise-robust training. We use continuous rather than discrete representations to retain prosody and speaker information. With this vocoding task alone, the model can perform speech enhancement better than a masking-based baseline. We further fine-tune the diffusion model on clean/noisy utterance pairs to improve the performance. Our approach outperforms a masking-based baseline in terms of both automatic metrics and a human listening test and is close in quality to the target speech in the listening test. Audio samples can be found at https://home.ttic.edu/~jcchou/demo/avse/avse_demo.html.

==> cmos_backup.tex <==
\begin{table}[htbp]
\begin{center}
\begin{tabular}{llr}
\toprule
       \multicolumn{1}{c}{Approach}       & \multicolumn{1}{c}{Other}        & \multicolumn{1}{c}{CMOS}              \\ \midrule
      AV2Wav-23-long-avse        & Baseline~\cite{blanco2023avse}          &    2.23 $\pm$ 0.18                    \\ \hline
      AV2Wav-23-long-avse        & AV2Wav-23-long          &    0.24 $\pm$ 0.20                    \\ \hline
        AV2Wav-23-long-avse        & Target          &    -0.53 $\pm$ 0.26                    \\ \hline
        AV2Wav-23-long re-syn        & Target          &    -0.17 $\pm$ 0.22             \\ \bottomrule

\end{tabular}
\end{center}
\caption{CMOS results for AV2Wav with 95\% confidence interval. \textit{AV2Wav-23-long re-syn} refers to the re-synthesized waveform using \textit{AV2Wav-23-long}.}
\label{tab:cmos_backup}
\end{table}

==> fast.tex <==
\begin{table}[htbp]
\begin{center}
\begin{tabular}{l|rr}
\toprule
              & WER        & P-SI-SDR              \\ \midrule
AV2Wav-cont-100  &   17.46         &    18.43               \\ \hline
AV2Wav-ddim-100  &   16.21         &    18.17                  \\ \midrule
AV2Wav-ddim-50      &      15.73      &      18.15                 \\ \hline
AV2Wav-ddim-25      &      16.41      &      17.58                 \\ \bottomrule
\end{tabular}
\label{tab:fast}
\end{center}
\caption{WER and predicted SI-SDR (P-SI-SDR) by NQE with fast inference algorithm. The model variation is \textit{AV2Wav-23-long-avse}.}
\end{table}

==> fast_infer.tex <==
\begin{table}[htbp]
\begin{center}
\begin{tabular}{l|rr}
\toprule
              & WER        & P-SI-SDR              \\ \midrule
              \multicolumn{3}{c}{\textbf{Target re-synthesis}}   \\ \hline
              target  &   6.72         &    21.56                    \\ \hline
AV2Wav-23     &      3.15      &      21.36                 \\ \hline
AV2Wav-23-long     &      \textbf{2.71}      &      \textbf{22.24}                 \\ \hline
AV2Wav-25     &     3.00       &          21.76         \\ \hline
AV2Wav-random &     2.94       &      19.79                 \\ \hline
\multicolumn{3}{c}{\textbf{Mixed speech}}   \\ \hline
mixed  &   48.45         &    0.12               \\ \hline
AVSE-baseline~\cite{blanco2023avse}  &   26.40         &    13.79                  \\ \hline
VisualVoice*~\cite{gao2021visualvoice}  &   44.61         &    2.80                  \\ \midrule
AV2Wav-23     &      18.17      &      19.41                 \\ \hline
AV2Wav-23-long     &      17.20      &      20.09                 \\ \hline
AV2Wav-25     &     17.36       &          20.07          \\ \hline
AV2Wav-random &     19.69       &      14.57                  \\ \midrule
\multicolumn{3}{c}{\textbf{After fine-tuning}}   \\ \hline
AV2Wav-23-avse     &      \textbf{15.85}      &      20.65            \\ \hline
AV2Wav-23-long-avse     &      16.76      &      21.21               \\ \hline
AV2Wav-23-vctk     &      16.71      &      \textbf{21.79}                  \\ \hline
AV2Wav-23-avse-vctk     &      16.90       &      19.96           \\ \hline
\multicolumn{3}{c}{\textbf{Fast inference}}   \\ \hline
AV2Wav-cont-100  &   17.46         &    18.43               \\ \hline
AV2Wav-ddim-100  &   16.21         &    18.17                  \\ \hline
AV2Wav-ddim-50      &      15.73      &      18.15                 \\ \hline
AV2Wav-ddim-25      &      16.41      &      17.58                 \\ \bottomrule

\end{tabular}
\end{center}
\caption{WER and predicted SI-SDR (P-SI-SDR) by NQE on mixed speech (speech + interferer). For fast inference, we use \textit{AV2Wav-23-long-avse}. (*) We use the source separation model and the speech enhancement model separately. The reason why the speech enhancement model performs poorly on our dataset should be further investigated. }
\label{tab:fast_infer}
\end{table}

==> target.tex <==
\begin{table}[htbp]
\begin{center}
\caption{WER and predicted SI-SDR (P-SI-SDR) by NQE on target re-synthesis. }
\begin{tabular}{l|rr}
\toprule
              & WER        & P-SI-SDR              \\ \midrule
target  &   6.72         &    21.56                    \\ \hline
AV2Wav-23     &      3.15      &      21.36                 \\ \hline
AV2Wav-23-long     &      \textbf{2.71}      &      \textbf{22.24}                 \\ \hline
AV2Wav-25     &     3.00       &          21.76         \\ \hline
AV2Wav-random &     2.94       &      19.79                 \\ \bottomrule
\end{tabular}
\label{tab:target}
\end{center}
\end{table}
